Identifying Crucial Objects in Blind and Low-Vision Individuals' Navigation

This paper presents a curated list of 90 objects essential for the navigation of blind and low-vision (BLV) individuals, encompassing road, sidewalk, and indoor environments. We develop the initial list by analyzing 21 publicly available videos featuring BLV individuals navigating various settings. Then, we refine the list through feedback from a focus group study involving blind, low-vision, and sighted companions of BLV individuals. A subsequent analysis reveals that most contemporary datasets used to train recent computer vision models contain only a small subset of the objects in our proposed list. Furthermore, we provide detailed object labeling for these 90 objects across 31 video segments derived from the original 21 videos. Finally, we make the object list, the 21 videos, and object labeling in the 31 video segments publicly available. This paper aims to fill the existing gap and foster the development of more inclusive and effective navigation aids for the BLV community.

==> sections/5.0.GT_labeling.tex <==
\section{Ground Truth Labeling and Dataset Analysis}
\label{sec:video_study}

To thoroughly analyze the collected videos, 
we split each video into small clips of variable lengths between five and ninety-five seconds.
%
Each clip revolves around the appearance of objects that are significant in people's navigation on roads and sidewalks.
We refer each clip to a video segment. Table~\ref{table:dataset} shows the number of segments created from each video. 
Using a keyframe extraction tool called \textit{Katna}\footnote{https://katna.readthedocs.io/en/latest/}, we further segmented the clips into keyframes. 
The keyframes are characterized as the representative frames of a video stream that serve a precise and concise summary of the video content, considering transitions in the scene and changes in lighting conditions and activities. 
% All the frames that appear between two successive keyframes compose a video clip. 
The number of keyframes (i.e., images) extracted from the video segments was between three and ninety-three. 
Afterward, we manually annotated the presence and absence of objects (of our final list) for a subset of keyframes extracted from the video segments. Let's denote the final list of objects as $L_u$ for future reference.
% Afterward, we manually generated ground-truth annotations for object recognition for every keyframe, encompassing all object categories that belong to $L_u$.

% \subsection{Ground Truth Labeling}
% All authors of this paper visually inspected the keyframes to generate ground truth. 
% Each author annotated a subset of video segments by observing the changes between two consecutive keyframes. 
% For each frame, the existence (denoted by 1) or absence (denoted by 0) of all the objects that belong to $L_{u}$ was annotated. 
% If In a keyframe $F_{k}$ the existence of the object $O \in L_{u}$ is denoted by a function $E$, the $E$ can be defined as follows:
% \[
%     E(O)= 
%     \begin{cases}
%         1,  & \text{if $O$ exists in $F_k$}\\
%         0,  & \text{otherwise}
%     \end{cases}
% \]
% Now the annotation of keyframe $F_k$ can be written as, $(E(O) \ | \ O \in L_u)$. 
% Since visually inspecting changes can be subject to ``\textit{change blindness}''---a phenomenon when the visual feed is momentarily interrupted by a blank screen~\cite{simons1997change}---we avoided this by viewing two consecutive keyframe pairs on the screen side-by-side and glancing between them. 

% For each video segment, annotating the first keyframe took the longest, typically 5-7 minutes. 
% For subsequent frames, we only looked at what objects newly appeared/disappeared from the previous frame and adjusted the annotations accordingly.
% Such differential annotation took less than 60 seconds in most cases. 
% The annotation task required more time if a new frame appeared with a completely different background or camera viewport. 
% With an average of around 15 keyframes per video segment, we needed around $\approx20$ minutes to annotate a video. 
% Each video segment was annotated by at least two researchers independently. 
% Later, we resolved the conflicts in annotation through collaboration. 

\subsection{Analyzing Annotated Data}
\label{subsec:analyzing_data}
Our annotation encompasses fine-grained object categories (belonging to $L_u$) with which people frequently interact while navigating an outdoor space. 
Some of these objects can create obstacles for people with visual impairment. Therefore, these objects are crucial for outdoor navigation for them. The bar chart in Figure~\ref{fig:dataset_stat} depicts the distribution of objects in our annotated dataset.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/dataset_dist.pdf}
    \caption{Bar chart representing the object distribution in our annotated data. Each bar represents the number of keyframes in which an object (as labeled on the x-axis) was present. 
    The X-axis also shows the id of the parent concept or group (as described in Table~\ref{table:taxonomy}) to which each object belongs. The Y-axis is in logarithmic scale.}
    \label{fig:dataset_stat}
\end{figure*}

According to our study findings, objects of some groups, such as ``\textit{Obstructions less likely to be detected by a white cane (group 3)}'', ``\textit{Objects that pick you before you pick them (group 5)}'', and  ``\textit{Objects not supposed to be on the sidewalk (group 7)}'' are considered as the most significant objects,
since failure in detecting these objects can cause accident or injury to blind people. As shown in Figure~\ref{fig:dataset_stat}, these objects appear in many keyframes of our collected videos. 
Therefore, Accurate detection of these objects is indispensable for blind navigation. 


AI models' readiness for blind navigation highly depends on their ability to correctly detect objects in our proposed list $L_u$ (also shown in Figure~\ref{fig:dataset_stat}). 
However, an object recognizer model can only recognize the objects that are present in its training dataset. 
In general, most Object recognition or detection models are trained on datasets such as ImageNet~\cite{deng2009imagenet}, MS COCO~\cite{lin2014microsoft}, Mapillary Vistas~\cite{neuhold2017mapillary}, Kitti~\cite{geiger2012we}, Cityscapes~\cite{cordts2016cityscapes}, Pascal VOC~\cite{everingham2010pascal}, PFB~\cite{pfb_ICCV2017}, and ADE20K~\cite{zhou2017scene, zhou2019semantic}.
%
Mapillary Vistas is the most advanced open-world dataset that contains high-resolution street-level images and fine-grained annotation of 66 outdoor object categories~\cite{neuhold2017mapillary}. Nevertheless, the ground-truth annotations of Mapillary Vistas and all the other datasets contain significantly fewer objects of our proposed list $L_u$. 
Additionally, these datasets hardly have annotations for the most significant objects---the ones from group 3, group 5, and group 7; shown within the first nine objects in Figure~\ref{fig:obj_existance} (from \textit{Bench} to \textit{Water Pipes}).
%
Figure~\ref{fig:obj_existance} shows a heatmap that represents the existence of object categories in some of the most prominent datasets, where 
\colorbox[HTML]{0000FF}{\phantom{x}} in a cell 
means the corresponding object exists in the corresponding dataset. 
In contrast, 
\colorbox[HTML]{D3D3D3}{\phantom{x}} means the object does not exist in the corresponding dataset. 

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/obj_existence.pdf}
    \caption{A heatmap representing the existence of different objects of our list $L_u$ in prominent datasets.}
    \label{fig:obj_existance}
\end{figure*}

From Figure~\ref{fig:obj_existance}, we can conclude that most of the objects from our list $L_u$ do not exist in the well-established datasets. 
The first nine objects (from bench to water pipes) from the left of the heatmap are the most significant objects (that belong to groups 3, 5, and 7). 
Only three of these objects exist in some datasets, such as Mapillary Vistas, ADE20K, ImageNet, and PFB.

==> sections/6.discussion.tex <==
\section{Discussion and Implications}
\label{sec:discussion}

% This section reflects on how to improve the overall quality of current computer vision models in object recognition for blind and low-vision people's navigation.
%

{\textbf{Incorporating accessibility information in existing datasets.}}
The small base dataset (Table~\ref{table:dataset}) and the comprehensive taxonomy (Table~\ref{table:taxonomy}) we generated can be propagated to any other existing datasets through ``few-shot'' learning~\cite{chen2017deeplab, tan2019efficientnet, bronskill2020tasknorm, finn2017model, vinyals2016matching, zintgraf2019fast}, where AI models can learn to perform VQA tasks on our base dataset. 
% 
Prior work has shown that blind and low-vision individuals can teach a machine (via few-shot learning) to achieve higher accuracy and robustness in real-world applications~\cite{kacorri2017people, lee2019revisiting}.
For example, blind individuals can teach a generic object recognizer to recognize personalized objects, such as their favorite mugs, white canes, or friends' cars, by providing a few, say 5-10, example images or videos of these objects~\cite{kacorri2017teachable}.
As such, our dataset can empower BLV individuals with personalized data-driven navigational technology. 


In addition, we can use the knowledge from this paper to understand the accessibility impact of individual objects on a scale of 1 to 5.
% 
In the future, we will use this knowledge to develop a deep-learning model that predicts the pixel-wise, contextualized accessibility impact within a scene.
Note that accessible labels are not necessarily the same as an object's name but contain useful and context-rich descriptions.
% 


{\textbf{Limitations.}}
Our work has notable limitations. First, we are unaware of the context in which the videos in our dataset were uploaded and whether these were well-rehearsed.
Second, most BLV individuals featuring the videos were experts in O\&M. 
Therefore, their information needs may differ from those not skilled in O\&M. 
Third, we only annotated the presence of 90 objects in each keyframe, which may be inadequate for some AI tasks, such as semantic segmentation.




% Mathematically, given that we have a base dataset with \{$I^{1}, I^{2}, ..., I^{N}$\} images and its corresponding pixel-wise semantic labels \{$S^{1}, S^{2}, ..., S^{N}$\}, where $N$ the total number of images. Each $k^{th}$ image $I^{k}$ with height $H$ and width $W$ contains color RGB values and its corresponding semantic segmentation $S^{k}$ contains labels from a fixed set of semantic categories \{$1, 2, ..., C$\}, where $C$ is the total number of semantic categories.
% \indent Our goal is to construct the set of accessibility labels for navigation \{$A^{1}, A^{2}, ..., A^{N}$\} and its corresponding 
% 
% In the end, this will enrich the existing semantic segmentation map $S^{k}$  of our base dataset with an additional map $accimpact^{k}$ for each image, $k$.


% \paragraph{\textbf{Develop a scalable algorithm to propagate accessibility impact labels from the base dataset to existing CV benchmark datasets}}
% % \paragraph{\textbf{Make existing datasets accessible by using semi-automated approach.}}
% High-quality semantic labeling involves a laborious, time-consuming, and costly human-annotation process~\cite{bearman_ECCV16, russakovsky_CVPR15}.
% For example, annotation of a single image might require 60-94 minutes depending on the complexity of the scene~\cite{playing_for_data_eccv16, cityscapes_cvpr16, mapiliary_iccv17}.
% A viable option to alleviate this laborious effort is to propagate labels either using a semi-automatic~\cite{reza_iros17, Marcu_2020_ACCV, marion_ICRA2018} or fully-automatic labeling approach~\cite{Reza_IROS19} on the video image sequences.
% To propagate information from one frame to another, the propagation method exploits the regularity in adjacent frames based on the optical-flow-based signal, camera trajectory, and 3D reconstructed models.
% However, transferring semantic labels from another relevant image is challenging for a standalone image.
% %
% In the future, we will develop new semi-automatic algorithms based on label-propagation to
% discover missing segments, such as \textit{e.g., curb-cut, ramps, crosswalk, snow} in existing dataset, as shown in Figure~\ref{fig:kitti15_dataset_sem}.

% \paragraph{\textbf{Transfer accessibility impact ratings from base dataset to any dataset}}

% Once the missing segments are discovered in an image, we investigate how to transfer the accessibility ratings to those segments from the base dataset. 
% One immediate challenge is that the distribution of ratings is likely to be imbalanced. 
% For example, segments afar like the sky, and clouds, are more frequent but likely to have a ``neutral'' accessibility impact. 
% % 
% Therefore, we will design algorithms and tools based on Human-AI collaboration. 


% We plan to release all of our code and data on GitHub.

==> sections/7.conlcusion.tex <==
% \section{Conclusion}
% While capable, current computer vision models are not yet suitable for direct use in navigation tasks for blind and low-vision individuals. 
% This is largely due to their lack of training on objects crucial for navigation in real-world scenarios. 
% To tackle this issue, we present a dataset comprising 90 objects vital for road navigation for blind and low-vision individuals. We refined this list through a focus group study involving both blind and low-vision individuals and sighted companions of blind individuals. 
% Additionally, we collected 21 navigational videos from publicly available sources and provided ground-truth labeling for 31 segments of these videos. 
% Our dataset fills a significant gap in existing datasets, which typically lack many of the objects crucial for navigation identified through our research. 
% This inadequacy is underscored by the subpar performance of seven state-of-the-art vision language models observed in our preliminary evaluation.
% By making our dataset publicly available, we aim to facilitate the retraining and enhancement of existing computer vision models for real-time detection of road objects, ultimately improving navigation for blind and low-vision individuals.





% Despite the immense capabilities of recent computer vision models in real-time object detection, they are not quite ready to be used by blind and low-vision users directly in their navigation tasks yet because, in most cases, they are not trained on many necessary objects that such users want to be detected.
% To address this issue, we propose a dataset with 90 accessibility-focused objects that are crucial to road navigation for blind and low-vision users.
% Our list of objects is refined through a focus group study with blind and low-vision users as well as sighted companions of blind users.
% We also provide 21 navigational videos collected from publicly available platforms and ground truth labeling for 31 video segments from these 21 videos and make the dataset publicly available.
% Deeper analysis indeed shows that most current datasets contain only a small subset of the objects we identified and proposed in the dataset.
% This is further validated by the relatively poor performance of eight state of the art vision language models in a preliminary study.
% Our proposed dataset can be used to retrain and improve the prediction performance of computer vision algorithms for real-time detetcion of road objects and improve navigation  for blind and low-vision users.


















% \fx{Assigned: Reza}
% In this paper, we assessed the robustness of two state-of-the-art VQA models on video frames of blind and low-vision users navigating around public places. 
% We collected videos from public video platforms, created a list of 90 crucial objects in the accessibility of roads for blind and low-vision users, and then built a dataset of as many questions concerning these objects. 
% Experimentally, we found that the selected VQA models (GPV-1 and BLIP) are vulnerable to practical use by people with blindness and low vision as they struggle to answer the questions in our proposed dataset. 
% We illustrated that the tested VQA models exhibit sequential-frame answer inconsistency, where their answers to our dataset's questions differ significantly despite the visual information across two frames remaining nearly identical.
% To address these issues, we provide recommendations on polishing the current VQA models for accessibility and incorporating accessibility information in large-scale datasets.

 

==> sections/ai_model_evaluation_old.tex <==
\section{Preliminary Evaluations on the Dataset}
\label{sec:assessing_vqa_models}

We picked \textbf{eight} state-of-the-art Vision Language Models (VLM) and tested them on our dataset.
More specifically, we tested how well these models could identify the objects in our taxonomy (Table~\ref{table:taxonomy}) in different video frames within our dataset.
%
These models provide solutions to various tasks, such as image captioning, object localization, image descriptions, and visual question answering (VQA)~\cite{gupta2022gpv}. 

For our purpose, we only focused on the VQA module of all models.
%
The models we chose are i) GPV-1~\cite{Gupta2021GPV} (\textit{general purpose vision} model), ii) BLIP~\cite{li2022blip} (available under the LAVIS~\cite{li2022lavis} package), iii) GPT-4~\cite{openai2023gpt4,openai2023gpt4vsc,openai2023gpt4vtwa},
iv) RAM (Recognize Anything Model)~\cite{zhang2023recognize}, 
v) Faster\_R-CNN~\cite{ren2015faster},
vi) YOLO\_V7~\cite{wang2023yolov7}, 
vii) HRNet\_V2~\cite{wang2020deep2}, and
viii) Mask\_R-CNN~\cite{he2017mask}.



% \subsection{Experiments and Observations}

\textbf{Experiment Procedure.}
Traditionally, visual questions are formed from broad categories of question types such as (i) recognition, (ii) common sense, (iii) reasoning, (iv) OCR, and (v) counting. 
State-of-the-art VQA models tend to perform well when asked visual recognition questions; however, these models are prone to failure when asked from other question categories~\cite{li2021adversarial}. 
%
To test our selected models, we asked simple visual recognition questions. 
We generated a set of questions, each focusing on one accessibility-related object as shown in Table~\ref{table:taxonomy}. 
All of our questions followed a predominant structure like ``Is there object X in the scene?'', where X is an object that came from Table~\ref{table:taxonomy}. 
Consequently, the answer from the VQA model was either ``yes'' or ``no''.

We also asked some other questions where the answer was neither simple ``yes'' nor ``no''.
For instance, in addition to asking a VQA model if there is a person with a disability in the scene, we also asked what kind of disability the person has.
% In addition, we also tested the impact of image quality on the model's capability.
%
% \textbf{Observations from VQA Outputs.}
We noticed that all of the tested models could correctly detect whether a white cane or a person with a disability was on the scene in most cases. 
However, they failed to answer what type of disability (e.g., blindness or vision impairment) the person has. 
This is not surprising and can be explained by the lack of representative annotations in the datasets.



% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/gallery.pdf}
%     \caption{Captured key frames from a short video segment (from V15 in Table~\ref{table:dataset}) of a blind person walking on a road. The numbers at the top-left corner represent the sequences of the frames. 
%     For all 15 frames (numbered from 0-14), the responses of two state-of-the-art VQA models to our questionnaire are shown in Figure~\ref{fig:vqa_outputs_no_GT}. Comparisons of these responses to ground truth are shown in Figure~\ref{fig:comp_GT}.}
%     \label{fig:gallery}
% \end{figure*}


% \textbf{Observations from Visualizations (No Ground Truth).}
% We found the two VQA models to be sensitive to minor changes in the camera viewport, despite very few (next-to-none in most cases) changes in the image content.
% This phenomenon is depicted in Figures~\ref{fig:gallery} and ~\ref{fig:vqa_outputs_no_GT}. 

% From Figure~\ref{fig:gallery}, we can visually inspect the minimal changes between two consecutive frames in most cases, unless there is a completely new scene like the transition from Frame-11 to Frame-12.
% However, both VQA models had a tendency to change their responses drastically even for two very similar frames, displaying their lack of reliability and general inconsistency.
% This inconsistency can be observed in Figure~\ref{fig:vqa_outputs_no_GT} by comparing two consecutive frames (i.e., columns), captures of which are shown in Figure~\ref{fig:gallery}. 
% From Figure~\ref{fig:vqa_outputs_no_GT}, we can see that the model on the left (GPV-1) is more inconsistent than the model on the right (BLIP~\cite{li2022blip}) in this regard.

% Moreover, we found the two models to be sensitive to image quality and lighting conditions.
% As such, we excluded some video segments (i.e., sequence of frames) where human eyes (i.e., ground truth annotators) struggle to detect an object and answer our set of questions.



% \begin{figure*}[!ht]
%     \begin{minipage}[t]{.45\textwidth}
%         \centering
%         \includegraphics[height=2.4\linewidth]{figures/gpv-GT-comp-15-3.pdf} \\
%         \hspace{55pt}
%         (a)~Model: GPV-1~\cite{Gupta2021GPV}
%     \end{minipage}
%     \hspace{-40pt}
%     \begin{minipage}[t]{.45\textwidth}
%       \centering
%         \includegraphics[height=2.4\linewidth]{figures/lavis-GT-comp-15-3.pdf} \\
%         \hspace{-70pt}
%         (b)~Model: BLIP~\cite{li2022blip} 
%     \end{minipage}
%     \caption{Performance of two VQA models (GPV-1~\cite{Gupta2021GPV} on the left, BLIP~\cite{li2022blip} on the right) based on their responses to our questionnaire, against ground truth. 
%     The video frames used for the evaluation  are numbered along the X-axis, while the Y-axis shows the objects in the center of a specific question.
%     The video frames are shown in Figure~\ref{fig:gallery}.}
%     \label{fig:comp_GT}
% \end{figure*}


\textbf{Comparison With Ground Truth.}
We compared the performance of the two models against our annotated ground truth data for 31 video segments as shown in Table~\ref{table:dataset}.
A short summary of the result reporting the precision, recall, F1-score, and accuracy is shown in Table~\ref{table:metric_summary}.

% The per-frame performance analyses of the two models for a specific video segment are shown in Figure~\ref{fig:comp_GT}; the frames of the video segment are shown in Figure~\ref{fig:gallery}.
% Our observation suggests that GPV-1 has a propensity towards producing a ``yes'' answer in case of confusion, which leads to a large number of false positives (see Figure~\ref{fig:gallery}a).
% The BLIP model, on the other hand, attempts to stick with ``no'' unless it has a certain degree of confidence about the existence of an object.


\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Model & Precision & Recall & F1 \\
 & (Micro Avg.) & (Micro Avg.) & (Micro Avg.) \\
\hline
\rowcolor{gray!10} 
GPT4V & 0.7365 & 0.6207 & 0.6737 \\
BLIP & 0.3366 & 0.8263 & 0.4783 \\
\rowcolor{gray!10} 
GPV-1 & 0.2273 & 0.8070 & 0.3547 \\
RAM & 0.8175 & 0.2715 & 0.4077 \\
\rowcolor{gray!10} 
YOLO\_V7 & 0.9437 & 0.1570 & 0.2692 \\
HRNet\_V2 & 0.6110 & 0.3998 & 0.4834 \\
\rowcolor{gray!10} 
Mask\_R-CNN & 0.6077 & 0.1801 & 0.2779 \\
Faster\_R-CNN & 0.6029 & 0.1837 & 0.2815 \\
\hline
\end{tabular}
\caption{Precision, Recall, and F1 scores for different models.}
\label{table:metric_summary}
\end{table}



% \subsection{Inter-Frame Similarity (IFS) Scores}
% \label{sec:IFS_scores}
% \begin{figure*}[t]
%     \centering
%     \begin{minipage}{.99\textwidth}
%         \centering
%         \includegraphics[width=1.0\textwidth]{figures/plots_frames/scatter_plot/scatter_plot_final.pdf}        
%     \end{minipage}
%     \caption{Scatter plots of Inter-Frame Similarity of human annotations vs others (IF, VQA1, and VQA2) at 5 different video segments.}
%     \label{fig:correlation_scatter_plot}
% \end{figure*}


% We visualize Inter-Frame Similarity (IFS) to facilitate rapid decision-making. 
% % Informed by these observations, we propose a human-centered approach to assess the reliability of VQA models. 
% The key idea is that if sighted humans observe two consecutive frames similarly, objects within these frames should likely be similar. 
% Therefore, an AI model is reliable if its calculated inter-frame similarity (IFS) score positively correlates with that of the sighted  humans' observations.
% The inter-frame similarity is widely used in video compression (e.g., MPEG) and motion trajectory predictions (e.g., Optical flow)~\cite{cai2021pedestrian}. 


% Let us denote an input video segment $\mathbf{S}$ containing $M$ consecutive keyframes or images. 
% That is, $\mathbf{S}$ = \{$I_1$, $I_2$, ..., $I_M$\}.
% % \reza{Reza: The following two lines are confusing hence I commented them out. Why these are important for our task?}
% %For each frame, $I_i$, we need to identify various foreground and background objects as well as their semantic instances. %Furthermore, we need to identify 3D spatial relationships between these objects, particularly the depth and motion flow, to describe inter-object relationships and the motion dynamics of different objects over multiple frames.
% Recall that IFS scores from sighted humans are available in our dataset as ground truth (Section~\ref{sec:dataset}).
% For AI models, we calculate two types of IFS scores: i) IFS of the Answers to Visual Questions and ii) feature-level IFS. 



% \textbf{IFS of the Answers to Visual Questions.}
% Based on our taxonomy of objects (Table~\ref{table:taxonomy}), we asked a fixed set $N$ of visual recognition questions for each image frame in a video sequence and construct a binary feature vector. 
% % 
% As shown in Figure~\ref{fig:comp_GT}, the first two questions are $Q_1$: \textit{Is there any Yard Waste in the scene?} and $Q_2$: \textit{Is there a white cane in the scene?}. 
% If the answers to these two questions are \textit{yes} while the remaining answers are \textit{no}, then the feature vector is represented by $[1, 1, 0, 0, 0, ..., 0]$. 
% A similar encoding method (i.e., the presence of different semantic categories arranged in a spatial pyramid) was used for a scene classification task in the work of~\cite{gupta_CVPR2013}.
% For frame $I_i$ and $I_{i+1}$, let us denote a VQA model's predicted answers by vectors $A_i$ and $A_{i+1}$, respectively. 
% For $N$ visual recognition questions %and the model answered the same for $n$ questions
% $QIFS(I_i, I_{i+1})$, the \textit{IFS of the Answers to Visual Questions}, is computed as follows:
% % \begin{equation}
% % % \[ 
% % QIFS(I_i, I_{i+1}) = \frac{n}{m} 
% % % \]
% % \end{equation}

% % \begin{equation}
% %  QIFS(I_i, I_{i+1})=
% %  \left\{\begin{matrix}
% %  n , & x_i=x_j\\
% %  m-n , & x_i\neq x_j,\\
% %  \end{matrix}\right.
% %  \end{equation}

%  \begin{equation}
%     QIFS(I_i, I_{i+1}) = \frac{1}{N} \sum_{j=1}^N{\mathbb{I}[A_{i}^j = A_{i+1}^j]}
% \end{equation}
% where $\mathbb{I}[.]$ is the \textit{Iverson bracket} -- an indicator function which produces 1 for true and 0 for false argument. $A_{i}^j$ denotes the $j^{th}$ element in vector $A_{i}$. Similarly, $A_{i+1}^j$ denotes the $j^{th}$ element in vector $A_{i+1}$. 
% In our experiments, we used two VQA models: i) GPV-1~\cite{gupta2022towards} and ii) BLIP~\cite{li2022blip}. 

% %about the existence of the classes mentioned in~\ref{table:taxonomy}. 
% % We asked a fixed set of visual recognition type VQA questions. Each visual recognition question is based on All the questions are arranged in a way that it can be answered in a binary format (\textit{yes} or \textit{no}). 

% \textbf{Feature-level IFS.}
% % \fx{This is the difference between features (the layer before the last layer. Pls expand: describe which models we used, rationale, and citations}
% For a given pair of consecutive image frames $I_i$ and $I_{i+1}$, the \textit{feature-level IFS} is based on their extracted deep feature maps.
% We used popular convolutional neural networks (CNN) such as AlexNet~\cite{krizhevsky2017imagenet}, VGG16~\cite{simonyan2014very}, and ResNet~\cite{he2016deep} for feature map extraction. 
% Each of these models contains a series of inner-product layers toward the end of the network. The last of these inner-product layers is the classification layer. We used the second last layer as our feature representation of an image.
% %By dropping the final layer from each model to extract features from images. 
% Lets consider the extracted features from images $I_i$ and $I_{i+1}$ are $F_i$ and $F_{i+1}$ respectively. We compute \textit{feature-level IFS} $FIFS(I_i, I_{i+1})$ by measuring cosine similarity between the feature vectors $F_i$ and $F_{i+1}$ as follows:
% % So, we can denote the feature level IFS $FIFS(I_i, I_{i+1})$ by,
% \begin{equation}
% % \[ 
% FIFS(I_i, I_{i+1}) = \frac{(F_i \cdot F_{i+1})}{\max({\Vert F_i \Vert}_2 \cdot {\Vert F_{i+1} \Vert}_2, \epsilon)} %\]
% \end{equation}

% where a small value of $\epsilon$ is used to avoid division by zero, and symbol $\cdot$ denotes the dot product between two feature vectors. 
% We computed IFS using four different models i.e. ResNet-152~\cite{he2016deep}, ResNet-52~\cite{he2016deep}, Alexnet~\cite{krizhevsky2017imagenet} and VGG-16~\cite{simonyan2014very}. From our experiments, we found that ResNet-152 based \textit{feature-level IFS} followed the trend of human annotation.

% % \paragraph{Class-level IFS}
% % \fx{This is the difference between class labels/object detection (the labels should come from benchmark datasets, such as IMAGENET, MSEG, and WildDASH. Pls expand.}
% % % 
% % Note ImageNet, MSEG, ... do not contain some objects or labels that are available in our taxonomy. Conversely, our taxonomy does not contain many labels from benchmark datasets because we only accessibility-related objects. In case a label does not exist, we \fx{did what?}.




% \begin{table*}[t]
% \centering
% \footnotesize
% % \resizebox{6.0cm}{!}{
% \begin{tabular}{c|c|rrl|rrl|rrl| rl | lll}
% \toprule
% \multirow{2}{*}{Video Seg.} & pairs & \multicolumn{3}{c}{Corr. GT vs Image Feat (IF)} & \multicolumn{3}{c}{Corr. GT vs VQA1 (GPV-1)} & \multicolumn{3}{c}{Corr. GT vs VQA2 (BLIP)} &  \multicolumn{2}{c}{ANOVA} & \multicolumn{3}{c}{paired t-tests}\\
% %& \cline{1-3} \\
% % Touhid: I created a third row in the header to fix the overflow problem. 
% & & $|r|$ & t & p-value  & $|r|$ & t & p-value  & $|r|$ & t & p-value & F-score & p-value & GT vs & GT vs & GT vs \\
% & &  &  &  &  &  &   &  &  &  &  &  & \multicolumn{1}{|c|}{IF} & \multicolumn{1}{|c|}{VQA1} & \multicolumn{1}{|c|}{VQA2} \\
% \midrule
% $V1_{S4}$ & 23 & \textbf{0.9309}  & 12.225 & .000 ***  & 0.4890 & 2.6885 & .013 *  & 0.6807 & 4.4567 & .000 ***  & 15.93 & .000 *** & .000 *** & .000 *** & .020 *  \\
% \hline
% \rowcolor{gray!10} 
% $V1_{S5}$ & 11 & \textbf{0.2891} & 1.0020 & .338 & 0.0555 & 0.1843 & .857  & 0.0785 & -0.2613 & .798 & 24.01 & .000 *** & .000 *** & .000 *** & .053 \\
% \hline
% $V2_{S1}$ & 45 & 0.7734 & 8.1856 & .000 *** & 0.6471 & 5.6941 & .000 ***  & \textbf{0.8156} & 9.4561 & .000 *** & 32.34 & .000 *** & .000 *** & .000 *** & .001 **\\
% \hline
% \rowcolor{gray!10} 
% $V3_{S2}$ & 9  & 0.5358 & 1.9037 & .089 & 0.1861 & 0.5682 & .584  & \textbf{0.7305} & 3.2092 & .011 * & 20.70 & .000 *** & .000 *** & .000 *** & .000 *** \\
% \hline
% $V3_{S3}$ & 53 & 0.2545 & 1.9160 & .061 & 0.0507 & -0.3693 & .713 & \textbf{0.4225} & 3.3934 & .001 ** & 73.10 & .000 *** & .000 *** & .000 *** & .000 ***\\
% \hline
% \rowcolor{gray!10} 
% $V4_{S1}$ & 11 & 0.3770 & 1.3501 & .204 & \textbf{0.7447} & 3.7008 & .003 **  & 0.1384 & 0.4635 & .652 & 14.25 & .000 *** & .000 *** &  .000 *** & .014 *\\
% \hline
% $V4_{S3}$ & 19 & \textbf{0.6578} & 3.8062 & .001 ** & 0.2701 & 1.2227 & .236  & 0.2846 & 1.2938 & .211 & 34.93 & .000 *** & .000 *** & .000 *** & .000 ***\\
% \hline
% \rowcolor{gray!10} 
% $V4_{S4}$ & 63 & \textbf{0.5289} & 4.9452 & .000 *** &  0.3182 & 2.6640 & .010 ** & 0.3914 & 3.3765 & .001 ** & 78.27 & .000 *** & 
% .000 *** & .000 *** & .000 ***\\
% \hline
% $V5_{S1}$ & 22 & \textbf{0.866}1 & 8.1264 & .000 *** & 0.5157 & 2.8233 & .010 **  & 0.8093 & 6.4618 & .000 *** &  32.20 & .000 *** & .000 *** & .000 *** & .030 *\\
% \hline
% \rowcolor{gray!10} 
% $V6_{S2}$ & 16 & 0.6040 & 3.0313 & .008 ** & 0.5463 & 2.6090 & .019 *  & \textbf{0.7542} & 4.5949 & .000 *** & 27.00 & .000 *** & .000 *** & .000 *** & .003 **\\
% \hline
% $V7_{S2}$ & 14 & 0.6805 & 3.4752 & .004 ** & 0.3791 & 1.5328 & .148 & \textbf{0.6869} & 3.5367 & .003 ** & 11.69 & .000 *** & .000 *** & .000 *** & .018 * \\
% \hline
% \rowcolor{gray!10} 
% $V8_{S2}$ & 32 & \textbf{0.5208} & 3.4507 & .002 ** & 0.1336 & 0.7626 & .451  & 0.0334 & 0.1891 & .851 & 103.70 & .000 *** & .000 *** & .000 *** & .000 ***\\
% \hline
% $V9_{S2}$ & 31 & \textbf{0.7305} & 5.9563 & .000 *** & 0.6006 & 4.1828 & .000 ***  & 0.4433 & 2.7535 & .009 ** & 29.00 & .000 *** & .000 *** & .000 *** & .000 ***\\
% \hline
% \rowcolor{gray!10} 
% $V10_{S1}$ & 17 & \textbf{0.7126} & 4.1884 & .000 *** & 0.6123 & 3.1933 & .005 ** & 0.6190 & 3.2494 & .004 ** & 17.24 & .000 *** & .000 *** & .000 *** & .040 *\\
% \hline
% $V11_{S1}$ & 17 & \textbf{0.8344} & 6.2414 & .000 *** & 0.7883 & 5.2825 & .000 *** & 0.8145 & 5.7875 & .000 *** & 14.29 & .000 *** & .055 & .000 *** & .320 \\
% \hline
% \rowcolor{gray!10} 
% $V12_{S4}$ & 21 & \textbf{0.8843} & 8.6794 & .000 *** & 0.4232 & 2.1406 & .044 * & 0.7811 & 5.7330 & .000 *** & 13.49 & .000 *** & .000 *** & .000 *** & .650 \\
% \hline
% $V13_{S2}$ & 24 & 0.6121 & 3.7923 & .000 *** & 0.3585 & 1.8814 & .072 & \textbf{0.6728} & 4.4548 & .000 *** & 11.42 & .000 *** & .000 *** & .000 *** & .200 \\
% \hline
% \rowcolor{gray!10} 
% $V14_{S1}$ & 12 & 0.8022 & 4.6545 & .000 *** & 0.9270 & 8.5657 & .000 *** & \textbf{0.9484} & 10.3600 & .000 *** & 8.77 & .000 *** & .000 *** & .000 *** & .130 \\
% \hline
% $V14_{S4}$ & 9  & 0.8236 & 4.3561 & .002 ** & 0.8060 & 4.0858 & .002 ** & \textbf{0.8418} & 4.6782 & .001 ** & 3.15 & .035 * & .082 & .059 & .825 \\
% \hline
% \rowcolor{gray!10} 
% $V15_{S3}$ & 12 & \textbf{ 0.7871} & 4.4196 & .000 *** & 0.1051 & 0.3661 & .720 & 0.6167 & 2.7133 & .019 * & 27.73 & .000 *** & .000 *** & .000 *** & .013 * \\
% \hline
% $V16_{S3}$ & 9  & 0.7879 & 3.8390 & .004 ** & 0.8970 & 6.0894 & .000 *** & \textbf{0.9209} & 7.0899 & .000 *** & 5.73 & .002 ** & .070 & .001 ** & .473 \\
% \hline
% \rowcolor{gray!10} 
% $V17_{S1}$ & 8  & \textbf{0.9336} & 0.2652 & .798 & 0.1981 & 0.5717 & .583 & 0.4883 & -1.5825 & .152 & 37.35 & .000 *** & .000 *** & .000 *** & .003 ** \\
% \hline
% $V17_{S3}$ & 30 & \textbf{0.8323 }& 8.2245 & .000 *** & 0.7383 & 5.9957 & .000 *** & 0.6450 & 4.6236 & .000 *** & 17.95 & .000 *** & .000 *** & .000 *** & .005 ** \\
% \hline
% \rowcolor{gray!10} 
% $V18_{S1}$ & 18 & \textbf{0.5966} & 3.1541 & .006 ** & 0.4698 & 2.2576 & .037 * & 0.4639 & 2.2218 & .039 * & 23.55 & .000 *** & .000 *** & .000 *** & .000 *** \\
% \hline
% $V18_{S6}$ & 11 & \textbf{0.9078} & 7.1776 & .000 *** & 0.4406 & 1.6280 & .131 & 0.6635 & 2.9418 & .013 * & 6.91 & .000 *** & .000 *** & .006 ** & .008 ** \\
% \hline
% \rowcolor{gray!10} 
% $V19_{S2}$ & 14 & 0.7495 & 4.2361 & .000 *** & 0.3374 & 1.3411 & .201 & \textbf{0.9107} & 8.2476 & .000 *** & 4.89 & .004 ** & .007 ** & .014 * & .399 \\
% \hline
% $V19_{S4}$ & 6 & \textbf{0.7134} & 2.4937 & .050 * & 0.2799 & 0.7143 & .500 & 0.6461 & 2.0735 & .080 & 5.54 & .004 ** & .018 * & .010 * & 1.00 \\
% \hline
% \rowcolor{gray!10} 
% $V20_{S1}$ & 4 & 0.4779 & -1.0881 & .337 & 0.2286 & 0.4697 & .663 & \textbf{0.5573} & -1.3425 & .251 & 16.35 & .000 *** & .055 & .000 *** & .235\\
% \hline
% $V20_{S5}$ & 2 & \textbf{0.9008} & -3.0723 & .092 & 0.0967 & 0.1374 & .903 & 0.1690 & 0.2425 & .831 & 18.34 & .000 *** & .219 & .000 *** & .049 *\\
% \hline
% \rowcolor{gray!10} 
% $V21_{S1}$ & 3 & \textbf{0.9912} & 13.006 & .000 *** & 0.7847 & 2.1924 & .116 & 0.5899 & 1.2654 & .295 & 8.32 & .001 ** & .020 * & .001 ** & .207\\
% \hline
% $V21_{S5}$ & 12 & 0.8355 & 5.2669 & .000 *** & 0.8479 & 5.5398 & .000 *** & \textbf{0.9246} & 8.4052 & .000 *** & 5.81 & .002 ** & .403 & .001 ** & 1.00\\
% \bottomrule
% \end{tabular}
% % }
% \caption{The correlation of inter-frame similarity scores between ground-truth (GT) vs. image-based feature, ground-truth (GT) vs. VQA (GPV-1), and ground-truth (GT) vs VQA (BLIP).}
% \label{table:evaluation_correlation_table}
% \end{table*}

\begin{comment}
    


\subsection{Evaluation}
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC374386/
% https://statsandr.com/blog/how-to-do-a-t-test-or-anova-for-many-variables-at-once-in-r-and-communicate-the-results-in-a-better-way/

\subsubsection{Correlation analysis}
\label{sec:r}
% 
We investigated how the similarity scores of two VQA models correlate with ground truth (GT). 
If the VQA models strongly (positively) correlate with GT, the correlation ($r$) should be close to $1$. 
On the other hand, $r$ values close to $0$ indicate that the similarity scores of VQA models can be random and noisy. 

Since an arbitrary video segment is unlikely to have ground truth, we explored whether GT can be approximated by other readily available measures, image-based features (IF). 
Therefore, we report a third correlation between GT and Image Feat. 
Table~\ref{table:evaluation_correlation_table} presents these measures. 

% \fx{Explain: 
% We notice that most correlation values are over $0.5$;  between GT and IF, these values are as high as 0.9. Most correlations are statistically significant. We can also observe that these values are consistent and do no varies like the correlation values of GT and VQA1, which means IF more closely follows the GT trend. The correlation values between GT and VQA1 are not consistent and varies significantly from video segment to segment. Most of the cases the correlation values are less than $0.5$, which means these correlations are statistically less significant. From the correlation values of GT and VQA2 we can notice that, these values are higher than the values of VQA1. However, correlation values between GT and VQA2 often jumps drastically from high to low values. Which means we can not fully rely on the Answers to VQA2 even if its correlation values are higher than the VQA1 correlation values.} 

We notice that most correlation values are over $0.5$;  between GT and IF (Image Feature), these values are as high as 0.9. 
Most correlations are statistically significant. 
We also observe that these values (GT and IF) are consistent and do not vary like the correlation values of GT and VQA1 (GPV-1), 
meaning IF more closely follows the GT trend. 
The correlation values between GT and VQA1 are inconsistent and vary significantly in different video segments. 
In most cases, the correlation values are less than $0.5$; and the correlations are not statistically significant. 
From the correlation values of GT and VQA2, we can notice that these values are higher than the values of VQA1, implying VQA2 is more robust than VQA1. 
This correlation gap (between VQA2 and VQA1) could be attributed to the large-scale pre-training, which the VQA2 model went through with additional noisy image-text pairs collected from the internet~\cite{li2022blip}. 
However, correlation values between GT and VQA2 (BLIP) exhibit drastic variation in Table~\ref{table:evaluation_correlation_table}. Hence answers from VQA2 are unreliable even if their correlation values are higher than the VQA1 correlation values. 
Figure ~\ref{fig:correlation_scatter_plot} shows the correlation between GT and other variables (IF, VQA1, and VQA2) in terms of Inter-frame Similarity (IFS) scores for 5 different video segments.

\subsubsection{ANOVA analysis}
We also conducted ANOVA analyses for each video segment where the dependent variable is the IFS score and the independent variable has four factors: GT, IF, VQA1, and  VQA2. 
Through ANOVA analysis, we compute the F-score and the P-value of the F statistic. The P-value represents the statistical significance of the variables. If P-value is less than $0.001$, then we can say that the variables have higher statistical significance. 
From ANOVA analysis, we can determine the overall significance of the variables, but we can not determine which pairs of variables are more statistically significant. 
So, we ran a pairwise test with the Bonferroni P-value adjustment method to determine how significant each pair of variables is. In the rightmost column of Table~\ref{table:evaluation_correlation_table}, the P-values of (GT, IF), (GT, VQA1), and (GT, VQA2) pairs are presented.



%The F value column is the test statistic from the F test. This is the mean square of each independent variable divided by the mean square of the residuals. The larger the F value, the more likely it is that the variation caused by the independent variable is real and not due to chance.%

%The Pr(>F) column is the p value of the F statistic. This shows how likely it is that the F value calculated from the test would have occurred if the null hypothesis of no difference among group means were true.%



\end{comment}

